Pifthon: A Compile-Time Information Flow Analyzer For An Imperative Language

Compile-time information flow analysis has been a promising technique for protecting confidentiality and integrity of private data. In the last couple of decades, a large number of information flow security tools in the form of run-time execution-monitors or static type systems have been developed for programming languages to analyze information flow security policies. However, existing flow analysis tools lack in precision and usability, which is the primary reason behind not being widely adopted in real application development. In this paper, we propose a compile-time information flow analysis for an imperative program based on a hybrid (mutable + immutable) labelling approach that enables a user to detect information flow-policy breaches and modify the program to overcome violations. We have developed an information flow security analyzer for a dialect of Python language, PyX, called Pifthon using the said approach. The flow-analyzer aids in identifying possible misuse of the information in sequential PyX programs corresponding to a given information flow policy (IFP). Pifthon has distinct advantages like reduced labelling overhead that ameliorates usability, covers a wide range of PyX programs that include termination-and progress-sensitive channels, in contrast to other approaches in the literature. The proposed flow analysis is proved to be sound under the classical non-interference property. Further, case study and experience in the usage of Pifthon are provided.

==> background.tex <==
\section{Background}
\label{sec:background}
In this section, we provide a brief overview of the Readers-Writers Flow Model ({\tt RWFM}) \cite{kumar2017complete,kumar2014realizing,narendra2015poster} for information flow control, followed by the definition of flow security for a program, and various labelling schemes adapted in the existing literature.

\subsection{Readers-Writers Flow Model(\texttt{RWFM}): An Overview}
\label{subsec:rwfm}
\begin{defn}[Readers-Writers Flow Model]   
\texttt{RWFM} model is defined as an eight tuple $(S,O,SC,\leqslant,\oplus,\otimes,\top,\bot)$, where $S$ and $O$ are the set of subjects and objects in the system, $SC=S\times2^S\times 2^S$ is the set of labels, $\leqslant=(-,\supseteq,\subseteq)$ is the permissible flows ordering (read as \textit{can-flow-to}), $\oplus=(-,\cap,\cup)$ and $\otimes=(-,\cup,\cap)$ are the join and meet operators respectively, and $\top=(-,\emptyset,S)$ and $\bot=(-,S,\emptyset)$ are respectively the maximum and minimum elements.
\end{defn}

\noindent Note that, $(SC,\leqslant,\oplus,\otimes)$ forms a lattice, where $(SC,\leqslant)$ is a partially ordered set. Let us define the labelling function $\lambda$ which maps a subject/object to its respective security label in $SC$, i.e., $\lambda: S\cup O\rightarrow SC$. A \texttt{RWFM} label ($SC=S\times2^S\times 2^S$) of a subject/object is written in the format: (Owner/Authority, \{Readers\}, \{Writers/Influencer\}). The component \textit{owner} represents the keeper of the information, the \textit{readers} component denotes the set of subjects allowed to read the information, and finally the \textit{writers} component identifies the subjects who have influenced the information so far. For the sake of this paper, we limit our discussion on \texttt{RWFM} state transition rules within the \textit{read}, \textit{write}, and \textit{downgrading} only.

\begin{defn}[Read Rule]
\noindent{\it Subject $s$ with label $(s_1,R_1,W_1)$ requests read access to an object $o$ with label $(s_2,R_2,W_2)$}.\\
If $(s\in R_2)$ then\\
\indent change the label of $s$ to $(s_1,R_1\cap R_2,W_1\cup W_2)$\\
\indent ALLOW\\
Else\\
\indent DENY
\end{defn}

\begin{defn}[Write Rule]
\noindent{\it Subject $s$ with label $(s_1,R_1,W_1)$ requests read access to an object $o$ with label $(s_2,R_2,W_2)$}.\\
If $(s\in W_2\wedge R_1\supseteq R_2\wedge W_1\subseteq W_2)$ then\\
\indent ALLOW\\
Else\\
\indent DENY
\end{defn}

Note that in \texttt{RWFM}, as the information moves up in the lattice, the readers set continues to reduce, hence becomes more restrictive; whereas, writers set grows as more subjects contribute to the information.

\begin{defn}[Downgrading Rule]
\noindent{\it Subject $s$ with label $(s_1,R_1,W_1)$ requests to downgrade an object $o$ from its current label $(s_2,R_2,W_2)$ to $(s_3,R_3,W_3)$}.\\
If ($s \in R_2$ $\wedge$ $s_1=s_2=s_3$ $\wedge$ $R_1=R_2$ $\wedge$ $W_1=W_2=W_3$ $\wedge$ $R_2\subseteq R_3$ $\wedge$ ($W_1=\{s_1\}$ $\vee$ ($R_3-R_2\subseteq W_2$))) then\\
\indent ALLOW\\
Else\\
\indent DENY
\end{defn}

This says, \textit{the owner of an object can declassify the content to a subject only if that subject had influenced the information earlier.}

\subsection{Information-Flow Policy (IFP)}
\label{subsec:ifp}
As stated in Denning's Information Flow Model (DFM) \cite{denning1977certification} the necessary condition for the flow security of a program is: if there is information flow from object $x$ to $y$, denoted by $x\rightarrow y$, the flow is secure if $\lambda(x)\leqslant\lambda(y)$, where $\lambda$ is a labelling function defined previously. The condition is often referred to as the \textit{Information-Flow Policy} (IFP) that forms the basis for the program certification. A program is certified as flow secure if there are no violations of the flow policy at any program point during the execution.

\subsection{Classification of Labelling Mechanisms}
\label{subsec:labelling_schemes}
The outcome of information-flow certification mechanisms heavily depends on precise information-flow analysis. The precision may be defined as below:\\
\noindent Let $F$ be the set of all possible information flows in a system, and $A$ be the subset of $F$ authorized by a given IFP. Further, consider $E$ be the subset of $F$ ``executable'' given the flow control mechanisms in operation. The system is \textit{secure} if $E\subseteq A$, i.e., all executable flows are authorized. A secure system is \textit{precise} if $E=A$, i.e., all authorized flows are executable \cite{robling1982cryptography}.

The precision of information-flow analysis is contingent on distinct labelling mechanisms adapted in the current literature \cite{myers2001jif,russo2010dynamic,stefan2011flexible,zheng2007dynamic,buiras2014dynamic}. The labelling mechanism usually referred to the process of binding subjects and objects of a program with a security class (either statically or dynamically depending on the application) from the lattice of security classes. Each of the existing compile-time and run-time certification mechanisms chooses an object labelling method ranges over the classes outlined in Table \ref{table:label_classification}.

% \begin{wraptable}{Ri}{6cm}
\begin{table}[htb]
\centering
\caption{Classification of object labelling mechanisms for certification}
\label{table:label_classification}
\begin{tabular}{l|l|l}
\hline
\begin{tabular}{l}
{\bf pc Label}$\rightarrow$\\ \hline
{\bf Labelling}$\downarrow$
\end{tabular}
& {\bf Reset} & {\bf Monotonic}\\ \hline
{\bf Static} & $P_1$ & $P_2$\\ \hline
{\bf Dynamic} & $P_3$ & $P_4$\\ \hline
\end{tabular}
% \end{table}
\end{table}

The labelling mechanisms those belong to the classes $P_1$ or $P_2$ evaluate the objects' label a priori and refrain from altering the labels throughout the computation. Whereas, the mechanisms from classes $P_3$ and $P_4$ update the labels to accommodate flows from the object with higher security label, thus achieve \textit{flow-sensitivity} \cite{hunt2006flow}. In addition to that, the classes usually capture the implicit flows by tracking the progress of program counter ($pc$) whose label is either reset after every program statement ($P_1$, $P_3$) or updated monotonically ($P_2$, $P_4$). We compare subtle precisions in flow analysis captured by these classes through a lucid while-program in the next section.

% The method of binding security classes/labels to objects plays an important role in the analysis of programs. Each of the static certification and runtime enforcement algorithms proposed in the literature chooses an object labelling method, some of which may also use the label of the implicit variable, usually referred to as {\em program counter} (\texttt{pc}) which may be reset after every statement or keeps updating monotonically.

% $P_1$ and $P_2$ refer to the labelling mechanism where label of each object in a program is fixed or static over the course of the computation. The only difference with $P_1$ in the mechanism $P_2$ lets the label of \texttt{pc} to monotonically increase after executing each statement instead of resetting to the primary label. Therefore, at any program point the label of \texttt{pc} represents the \textit{upper bound} of all the labels the \texttt{pc} has observed so far. The mechanisms $P_3$ and $P_4$ allow to elevate the label of the object where information sinks from a higher labelled source, thus able to realize \textit{flow-sensitivity} \cite{hunt2006flow}, but likewise $P_2$, $P_4$ increases the label of \texttt{pc}.  











==> rwfm.tex <==
\section{Readers-Writers Flow Model(\texttt{RWFM})}
\label{sec:rwfm}
A brief overview of the Readers-Writers Flow Model (RWFM) \cite{kumar2017complete,kumar2014realizing,narendra2015poster} for information flow control is given here.
\begin{defn}[\textbf{RWFM Label}]
A \texttt{RWFM} label is a three-tuple $(s,R,W)$ ($s,R,W\in$ set of principals/subjects $P$), where $s$ represents the \textit{owner} of the information and policy, $R$ denotes the set of \textit{readers} allowed to read the information, and $W$ identifies the set of \textit{writers} who have influenced the information so far.
\end{defn}

\begin{defn}[\textbf{can-flow-to relation} ($\mathbf{\leqslant}$)]
Given any two \texttt{RWFM} labels $L_1=(s_1,R_1,W_1)$ and $L_2=(s_2,R_2,W_2)$, the can-flow-to relation is defined as:
\[
\dfrac{R_1\supseteq R_2\quad W_1\subseteq W_2}{L_1\leqslant L_2}
\]
\end{defn}

\begin{defn}[\textbf{Join and meet for RWFM Labels}]
The join ($\oplus$) and meet ($\otimes$) of any two \texttt{RWFM} labels $L_1=(s_1,R_1,W_1)$ and $L_2=(s_2,R_2,W_2)$ are respectively defined as
\[L_1\oplus L_2 = (-,R_1\cap R_2,W_1\cup W_2)\quad L_1\otimes L_2 = (-,R_1\cup R_2,W_1\cap W_2)\]
\end{defn}

\noindent The set of \texttt{RWFM} labels $SC=P\times2^P\times 2^P$ forms a bounded lattice $(SC,\leqslant,\oplus,\otimes,\top,\bot)$, where $(SC,\leqslant)$ is a partially ordered set and $\top=(-,\emptyset,P)$, and $\bot=(-,P,\emptyset)$ are respectively the maximum and minimum elements.

% \begin{defn}[Readers-Writers Flow Model]   
% \texttt{RWFM} is defined as an eight tuple $(S,O,SC,\leqslant,\oplus,\otimes,\top,\bot)$, where $S$ and $O$ are the set of subjects and objects in the system, $SC=S\times2^S\times 2^S$ is the set of labels, $\leqslant=(-,\supseteq,\subseteq)$ is the permissible flows ordering (read as \textit{can-flow-to}), $\oplus=(-,\cap,\cup)$ and $\otimes=(-,\cup,\cap)$ are the join and meet operators respectively, and $\top=(-,\emptyset,S)$ and $\bot=(-,S,\emptyset)$ are respectively the maximum and minimum elements.
% \end{defn}

% \noindent Note that, $(SC,\leqslant,\oplus,\otimes)$ forms a lattice, where $(SC,\leqslant)$ is a partially ordered set. Let us define the labeling function $\lambda$ which maps a subject/object to its respective security label in $SC$, i.e., $\lambda: S\cup O\rightarrow SC$. A \texttt{RWFM} label ($SC=S\times2^S\times 2^S$) of a subject/object is written in the format: (Owner/Authority, \{Readers\}, \{Writers/Influencer\}). The component \textit{owner} represents the keeper of the information, the \textit{readers} component denotes the set of subjects allowed to read the information, and finally the \textit{writers} component identifies the subjects who have influenced the information so far. For the sake of this paper, we limit our discussion on \texttt{RWFM} state transition rules within the \textit{read}, \textit{write}, and \textit{downgrading} only.

% \begin{defn}[Read Rule]
% \noindent{\it Subject $s$ with label $(s_1,R_1,W_1)$ requests read access to an object $o$ with label $(s_2,R_2,W_2)$}.\\
% If $(s\in R_2)$ then\\
% \indent change the label of $s$ to $(s_1,R_1\cap R_2,W_1\cup W_2)$\\
% \indent ALLOW\\
% Else\\
% \indent DENY
% \end{defn}

% \begin{defn}[Write Rule]
% \noindent{\it Subject $s$ with label $(s_1,R_1,W_1)$ requests read access to an object $o$ with label $(s_2,R_2,W_2)$}.\\
% If $(s\in W_2\wedge R_1\supseteq R_2\wedge W_1\subseteq W_2)$ then\\
% \indent ALLOW\\
% Else\\
% \indent DENY
% \end{defn}
% \vspace*{-0.10in}
% \noindent Note that in \texttt{RWFM}, as information moves up in the lattice, set of readers continues to reduce becoming more restrictive; whereas, writers' set grows as more subjects contribute to the information.

\begin{defn}[\textbf{Declassification in RWFM}]
\noindent{\it The declassification of an object $o$ from its current label $(s_2,R_2,W_2)$ to $(s_3,R_3,W_3)$} as performed by the subject $s$ with label $(s_1,R_1,W_1)$ is defined as
\[
\dfrac{\let\scriptstyle\textstyle\substack{s\in R_2\quad s_1=s_2=s_3\quad R_1=R_2\quad W_1=W_2=W_3\quad R_2\subseteq R_3\\(W_1=\{s_1\}\vee (R_3-R_2\subseteq W_2))}}{(s_2,R_2,W_2) \text{ may be declassified to }(s_3,R_3,W_3)}
\]
% If ($s \in R_2$ $\wedge$ $s_1=s_2=s_3$ $\wedge$ $R_1=R_2$ $\wedge$ $W_1=W_2=W_3$ $\wedge$ $R_2\subseteq R_3$ $\wedge$ ($W_1=\{s_1\}$ $\vee$ ($R_3-R_2\subseteq W_2$))) then\\
% \indent ALLOW\\
% Else\\
% \indent DENY
\end{defn}
\noindent This says, \textit{the owner of an object can declassify the content to a subject(s) only if the owner is the sole writer of the information or that subject(s) had influenced the information earlier.}

% \subsection{Classification of labeling Mechanisms}
% \label{subsec:labeling_schemes}


% The method of binding security classes/labels to objects plays an important role in the analysis of programs. Each of the static certification and runtime enforcement algorithms proposed in the literature chooses an object labeling method, some of which may also use the label of the implicit variable, usually referred to as {\em program counter} (\texttt{pc}) which may be reset after every statement or keeps updating monotonically.

% $P_1$ and $P_2$ refer to the labeling mechanism where label of each object in a program is fixed or static over the course of the computation. The only difference with $P_1$ in the mechanism $P_2$ lets the label of \texttt{pc} to monotonically increase after executing each statement instead of resetting to the primary label. Therefore, at any program point the label of \texttt{pc} represents the \textit{upper bound} of all the labels the \texttt{pc} has observed so far. The mechanisms $P_3$ and $P_4$ allow to elevate the label of the object where information sinks from a higher labelled source, thus able to realize \textit{flow-sensitivity} \cite{hunt2006flow}, but likewise $P_2$, $P_4$ increases the label of \texttt{pc}.  










